Efficient Neural Architecture for Text-to-Image Synthesis

Text-to-image synthesis is the task of generating images from text descriptions. Image generation, by itself, is a challenging task. When we combine image generation and text, we bring complexity to a new level: we need to combine data from two different modalities. Most of recent works in text-to-image synthesis follow a similar approach when it comes to neural architectures. Due to aforementioned difficulties, plus the inherent difficulty of training GANs at high resolutions, most methods have adopted a multi-stage training strategy. In this paper we shift the architectural paradigm currently used in text-to-image methods and show that an effective neural architecture can achieve state-of-the-art performance using a single stage training with a single generator and a single discriminator. We do so by applying deep residual networks along with a novel sentence interpolation strategy that enables learning a smooth conditional space. Finally, our work points a new direction for text-to-image research, which has not experimented with novel neural architectures recently.

==> Efficient Neural Architecture for Text-to-Image Synthesis/figures.tex <==
\newcommand{\figteaser}{
\newcommand{\h}{20.7mm}
\newcommand{\hh}{2.5mm}
\newcommand{\vv}{\vspace*{-0.35mm}}
\begin{figure}[t]
\centering
\begin{minipage}[c]{0.972\linewidth}
% \makebox[\hh][r]{}%
% \makebox[\hh][l]{}\hspace{0.5mm}%
\hspace{3.0mm}%
\parbox[c]{\h}{\centering \footnotesize{There is a red bird with black beady eyes and dark edged feather sitting on a branch.}}%
\parbox[r]{\h}{\centering \footnotesize{This is a small yellow bird with a grey head and\\a small pointy beak.}}%
\parbox[l]{\h}{\centering \footnotesize{A flower with thin long pink petals and central cluster of orange stamen.}}%
\parbox[l]{\h}{\centering \footnotesize{The petals of the flower are color yellow with red stripes.}}\vspace{2mm}\\
\makebox[\hh]{\rotatebox[origin=l]{90}{\hspace{-1.18mm}\makebox[\h][c]{\footnotesize{Ours}}}}\hspace{0.5mm}%
\includegraphics[height=\h]{figs/birds/teaser_bird1.png}%
\includegraphics[height=\h]{figs/birds/teaser_bird2.png}%
\includegraphics[height=\h]{figs/flowers/teaser_flower1.png}%
\includegraphics[height=\h]{figs/flowers/teaser_flower2.png}\vv\\
\makebox[\hh]{\rotatebox[origin=l]{90}{\hspace{-1.18mm}\makebox[\h][c]{\footnotesize{Ground Truth}}}}\hspace{0.5mm}%
\includegraphics[height=\h]{figs/birds/teaser_bird1_gt.png}%
\includegraphics[height=\h]{figs/birds/teaser_bird2_gt.png}%
\includegraphics[height=\h]{figs/flowers/teaser_flower1_gt.png}%
\includegraphics[height=\h]{figs/flowers/teaser_flower2_gt.png}\vv\\
\end{minipage}
\caption{\label{fig:teaser}%
Images generated by our method.
\vspace*{-1mm}
}
\end{figure}
}

%%%%%%%%%% comparative figs

\newcommand{\figbirds}{
\renewcommand{\h}{27.4mm}
\renewcommand{\hh}{2.5mm}
\renewcommand{\vv}{\vspace*{-0.35mm}}
\begin{figure*}[!t]
\centering
% \begin{minipage}[c]{0.972\linewidth}
\begin{minipage}[c]{167.4mm}
% \makebox[\hh][r]{}%
% \makebox[\hh][l]{}\hspace{0.5mm}%
\hspace{3.0mm}%
\parbox[c]{\h}{\centering \footnotesize{An entirely black bird with small yellow eyes and a short straight bill.}}%
\parbox[r]{\h}{\centering \footnotesize{A blue bird with black legs and a short pointed beak.}}%
\parbox[l]{\h}{\centering \footnotesize{This white colored bird has bright orange feet and a hint of orange in its beak.}}%
\parbox[l]{\h}{\centering \footnotesize{This is a small, yellow bird with black on the crown, nape, and wingbars.}}%
\parbox[l]{\h}{\centering \footnotesize{This is a brown bird with a white breast and a large beak.

}}%
\parbox[l]{\h}{\centering \footnotesize{This colorful bird has a red crown adn throat with a black eye ring, and a white and pink belly.
}}\vspace{2mm}\\
\makebox[\hh]{\rotatebox[origin=l]{90}{\hspace{-1.18mm}\makebox[\h][c]{\normalsize{StackGAN++}}}}\hspace{0.5mm}%
\includegraphics[height=\h]{figs/birds/compare_stackganv2_bird1.png}%
\includegraphics[height=\h]{figs/birds/compare_stackganv2_bird2.png}%
\includegraphics[height=\h]{figs/birds/compare_stackganv2_bird3.png}%
\includegraphics[height=\h]{figs/birds/compare_stackganv2_bird4.png}%
\includegraphics[height=\h]{figs/birds/compare_stackganv2_bird5.png}%
\includegraphics[height=\h]{figs/birds/compare_stackganv2_bird6.png}\vv\\
% \makebox[\hh][c]{}\hspace{0.5mm}%
\makebox[\hh]{\rotatebox[origin=l]{90}{\hspace{-1.18mm}\makebox[\h][c]{\normalsize{HDGAN}}}}\hspace{0.5mm}%
\includegraphics[height=\h]{figs/birds/compare_hdgan_bird1.png}%
\includegraphics[height=\h]{figs/birds/compare_hdgan_bird2.png}%
\includegraphics[height=\h]{figs/birds/compare_hdgan_bird3.png}%
\includegraphics[height=\h]{figs/birds/compare_hdgan_bird4.png}%
\includegraphics[height=\h]{figs/birds/compare_hdgan_bird5.png}%
\includegraphics[height=\h]{figs/birds/compare_hdgan_bird6.png}\vv\\
% \makebox[\hh][c]{}\hspace{0.5mm}%
\makebox[\hh]{\rotatebox[origin=l]{90}{\hspace{-1.18mm}\makebox[\h][c]{\normalsize{Ours}}}}\hspace{0.5mm}%
\includegraphics[height=\h]{figs/birds/compare_ours_bird1.png}%
\includegraphics[height=\h]{figs/birds/compare_ours_bird2.png}%
\includegraphics[height=\h]{figs/birds/compare_ours_bird3.png}%
\includegraphics[height=\h]{figs/birds/compare_ours_bird4.png}%
\includegraphics[height=\h]{figs/birds/compare_ours_bird5.png}%
\includegraphics[height=\h]{figs/birds/compare_ours_bird6.png}\vv\\
\end{minipage}
\caption{\label{fig:compare_birds}%
Qualitative results in the CUB Dataset.
\vspace*{-1mm}
}
\end{figure*}
}


\newcommand{\figflowers}{
\renewcommand{\h}{27.4mm}
\renewcommand{\hh}{2.5mm}
\renewcommand{\vv}{\vspace*{-0.35mm}}
\begin{figure*}[!t]
\label{fig:flowers}
\centering
\begin{minipage}[c]{167.4mm}
% \makebox[\hh][r]{}%
% \makebox[\hh][l]{}\hspace{0.5mm}%
\hspace{3.0mm}%
\parbox[c]{\h}{\centering \footnotesize{This flower has petals that are yellow and folded together.}}%
\parbox[r]{\h}{\centering \footnotesize{This flower features elongated pointed orange petals emanating out of the main bulb.}}%
\parbox[l]{\h}{\centering \footnotesize{The flower has petals that are purple and white with purple filaments.}}%
\parbox[l]{\h}{\centering \footnotesize{This flower is pink in color, and has petals that are striped.}}%
\parbox[l]{\h}{\centering \footnotesize{This flower has wide and very smooth white petals with yellow central accents.}}%
\parbox[l]{\h}{\centering \footnotesize{The petals of the flower are in various colors such as red, yellow, and purple.}}\vspace{2mm}\\
% \makebox[\hh]{\rotatebox[origin=l]{90}{\hspace{-1.18mm}\makebox[\h][c]{\normalsize{StackGAN}}}}\hspace{0.5mm}%
% \includegraphics[height=\h]{figs/birds/targan1.png}%
% \includegraphics[height=\h]{figs/birds/targan1.png}%
% \includegraphics[height=\h]{figs/birds/targan1.png}%
% \includegraphics[height=\h]{figs/birds/targan1.png}%
% \includegraphics[height=\h]{figs/birds/targan1.png}%
% \includegraphics[height=\h]{figs/birds/targan1.png}\vv\\
% \makebox[\hh][c]{}\hspace{0.5mm}%
\makebox[\hh]{\rotatebox[origin=l]{90}{\hspace{-1.18mm}\makebox[\h][c]{\normalsize{HDGAN}}}}\hspace{0.5mm}%
\includegraphics[height=\h]{figs/flowers/compare_hdgan_flower1.png}%
\includegraphics[height=\h]{figs/flowers/compare_hdgan_flower2.png}%
\includegraphics[height=\h]{figs/flowers/compare_hdgan_flower3.png}%
\includegraphics[height=\h]{figs/flowers/compare_hdgan_flower4.png}%
\includegraphics[height=\h]{figs/flowers/compare_hdgan_flower5.png}%
\includegraphics[height=\h]{figs/flowers/compare_hdgan_flower6.png}\vv\\
% \makebox[\hh][c]{}\hspace{0.5mm}%
\makebox[\hh]{\rotatebox[origin=l]{90}{\hspace{-1.18mm}\makebox[\h][c]{\normalsize{Ours}}}}\hspace{0.5mm}%
\includegraphics[height=\h]{figs/flowers/compare_ours_flower1.png}%
\includegraphics[height=\h]{figs/flowers/compare_ours_flower2.png}%
\includegraphics[height=\h]{figs/flowers/compare_ours_flower3.png}%
\includegraphics[height=\h]{figs/flowers/compare_ours_flower4.png}%
\includegraphics[height=\h]{figs/flowers/compare_ours_flower5.png}%
\includegraphics[height=\h]{figs/flowers/compare_ours_flower6.png}\vv\\
\end{minipage}
\caption{\label{fig:compare_flowers}%
Qualitative results in the Oxford-102 Dataset.
\vspace*{-1mm}
}
\end{figure*}
}


\newcommand{\figarithmetic}{
\renewcommand{\h}{22mm}
\renewcommand{\hh}{2.5mm}
\renewcommand{\vv}{\vspace*{-0.35mm}}
\begin{figure}[t]
\label{fig:vec_arithmetics}
\centering
\begin{minipage}[c]{68mm}
\parbox[c]{\h}{\centering \scriptsize{
$\phi (\mbox{``\textit{This is a}}$ \\ $\mbox{\textit{red bird}"})$
}}%
% \parbox[c]{3mm}{\centering \scriptsize{$-$}}%
\parbox[r]{\h}{\centering \scriptsize{$-$ \genfromtext{It is red}}}%
\parbox[l]{\h}{\centering \scriptsize{$+$ \genfromtext{It is blue}}}%
\makebox[\hh][t]{}\hspace{0.5mm}%
% \makebox[\hh][l]{}\hspace{0.5mm}%
\hspace{1.0mm}%
\includegraphics[height=\h]{figs/arithmetic/va_0_0.png}%
\hspace{1.0mm}%
\includegraphics[height=\h]{figs/arithmetic/va_1_0.png}%
\hspace{1.0mm}%
\includegraphics[height=\h]{figs/arithmetic/va_2_0.png}%
\hspace{1.0mm}%
\\
\vspace{1mm}
\parbox[t]{\h}{\centering \scriptsize{
     $\phi (\mbox{``\textit{Blue bird has}}$ \\ $\mbox{\textit{long beak}"})$
}}%
% \parbox[c]{3mm}{\centering \scriptsize{$-$}}%
\parbox[c]{\h}{\centering \scriptsize{$-$ \genfromtext{Long beak}}}%
\parbox[l]{\h}{\centering \scriptsize{$+$ \genfromtext{Small beak}}}%
\\
\includegraphics[height=\h]{figs/arithmetic/va_0_10.png}%
\hspace{1.0mm}%
\includegraphics[height=\h]{figs/arithmetic/va_1_10.png}%
\hspace{1.0mm}%
\includegraphics[height=\h]{figs/arithmetic/va_2_10.png}%
\\
\vspace{1mm}
\parbox[t]{\h}{\centering \scriptsize{
$\phi (\mbox{``\textit{White bird}}$ \\ $\mbox{\textit{long beak}"})$
}}%
\parbox[c]{\h}{\centering \scriptsize{$-$ \genfromtext{Red crown}}}%
\parbox[l]{\h}{\centering \scriptsize{$+$ \genfromtext{Black crown}}}%
\\
\includegraphics[height=\h]{figs/arithmetic/va_0_11.png}%
\hspace{1.0mm}%
\includegraphics[height=\h]{figs/arithmetic/va_1_11.png}%
\hspace{1.0mm}%
\includegraphics[height=\h]{figs/arithmetic/va_2_11.png}%
\end{minipage}
\caption{
Image generation based on condition space arithmetic of embedded textual descriptions.
\label{fig:regularities}
\vspace*{-1mm}
}
\end{figure}
}


\newcommand{\figarithmeticb}{
\renewcommand{\h}{27.4mm}
\renewcommand{\hh}{2.5mm}
\renewcommand{\vv}{\vspace*{-0.35mm}}
\begin{figure}[t]
\label{fig:vec_arithmetics}
\centering
\begin{minipage}[c]{\columnwidth}
% \makebox[\hh][r]{}%
% \makebox[\hh][l]{}\hspace{0.5mm}%
\makebox[\hh][c]{}\hspace{0.5mm}%
\makebox[\hh]{\rotatebox[origin=l]{90}{\hspace{-1.18mm}\makebox[\h][c]{}}}\hspace{0.5mm}%
\parbox[c]{\h}{\centering \footnotesize{\genfromtext{This is a red bird}}}%
% \parbox[c]{3mm}{\centering \footnotesize{$-$}}%
\parbox[r]{\h}{\centering \footnotesize{$-$ \genfromtext{It is red}}}%
\parbox[l]{\h}{\centering \footnotesize{$+$ \genfromtext{It is blue}}}%
\\
\includegraphics[height=\h]{figs/arithmetic/va_0_10.png}%
\hspace{1.0mm}%
\includegraphics[height=\h]{figs/arithmetic/va_1_10.png}%
\hspace{1.0mm}%
\includegraphics[height=\h]{figs/arithmetic/va_2_10.png}%
\end{minipage}
\caption{
Image generation based on condition space arithmetic of embedded textual descriptions.
\label{fig:regularities}
\vspace*{-1mm}
}
\end{figure}
}


\newcommand{\figarithmeticc}{
\renewcommand{\h}{27.4mm}
\renewcommand{\hh}{2.5mm}
\renewcommand{\vv}{\vspace*{-0.35mm}}
\begin{figure}[t]
\label{fig:vec_arithmetics}
\centering
\begin{minipage}[c]{\columnwidth}
\parbox[c]{\h}{\centering \footnotesize{\genfromtext{This is a red bird}}}%
% \parbox[c]{3mm}{\centering \footnotesize{$-$}}%
\parbox[r]{\h}{\centering \footnotesize{$-$ \genfromtext{It is red}}}%
\parbox[l]{\h}{\centering \footnotesize{$+$ \genfromtext{It is blue}}}%
\\
\makebox[\hh][c]{}\hspace{0.5mm}%
\makebox[\hh]{\rotatebox[origin=l]{90}{\hspace{-1.18mm}\makebox[\h][c]{}}}\hspace{0.5mm}%
\includegraphics[height=\h]{figs/arithmetic/va_0_11.png}%
\hspace{1.0mm}%
\includegraphics[height=\h]{figs/arithmetic/va_1_11.png}%
\hspace{1.0mm}%
\includegraphics[height=\h]{figs/arithmetic/va_2_11.png}%

\end{minipage}
\caption{
Image generation based on condition space arithmetic of embedded textual descriptions.
\label{fig:regularities}
\vspace*{-1mm}
}
\end{figure}
}
